Efficient Training for Positive Unlabeled Learning

Positive unlabeled (PU) learning is useful in various practical situations, where there is a need to learn a classifier for a class of interest from an unlabeled data set, which may contain anomalies as well as samples from unknown classes. The learning task can be formulated as an optimization problem under the framework of statistical learning theory. Recent studies have theoretically analyzed its properties and generalization performance, nevertheless, little effort has been made to consider the problem of scalability, especially when large sets of unlabeled data are available. In this work we propose a novel scalable PU learning algorithm that is theoretically proven to provide the optimal solution, while showing superior computational and memory performance. Experimental evaluation confirms the theoretical evidence and shows that the proposed method can be successfully applied to a large variety of real-world problems involving PU learning.

==> closeness.tex <==
\externaldocument{src/puformulation}
\todo{}

==> doublehinge.tex <==
\externaldocument{src/puformulation}
\subsection{Derivation of the primal problem}
By taking into account the definition of the double Hinge loss function and its composite loss, namely $\ell(x,y)=\max\{-xy,\max\{0,\frac{1}{2}-\frac{xy}{2}\}\}$ and $\tilde{\ell}(x,y)=-xy$, we can express the empirical risk functional~(\ref{eq:emprisk}) in the following way:
%
%
{\small\begin{equation}
\label{eq:doublerisk}
-\frac{\pi}{p}\sum_{i:\bm{x}_i\in D_p}f(\mathbf{x}_i)+\frac{1}{n}\sum_{i:\bm{x}_i\in D_n}\max\bigg\{f(\mathbf{x}_i),\max\big\{0,\frac{1}{2}+\frac{f(\mathbf{x}_i)}{2}\big\}\bigg\}
\end{equation}}
%
%
and by exploiting the result stated by the representer theorem, the optimization problem~(\ref{eq:puopt}) becomes:
%
%
{\small\begin{align}
\label{eq:doubleobj}
\min_{\bm{\alpha},\bm{\xi},\beta}&\:\bigg\{{-}c_1\sum_{i:\bm{x}_i\in D_p}\Bigg(\sum_{j:\bm{x}_j\in D}\alpha_j k(\mathbf{x}_i,\mathbf{x}_j)+\beta\Bigg)+c_2\sum_{i:\bm{x}_i\in D_n}\xi_i\nonumber\\
&\:+\frac{1}{2}\sum_{i:\bm{x}_i\in D}\sum_{j:\bm{x}_j\in D}\alpha_i\alpha_jk(\mathbf{x}_i,\mathbf{x}_j)\bigg\}\nonumber\\
\text{s.t.}&\;\xi_i\geq 0,\nonumber\\
&\:\xi_i\geq\sum_{j:\bm{x}_j\in D}\alpha_j k(\mathbf{x}_i,\mathbf{x}_j)+\beta,\nonumber\\
&\:\xi_i\geq\frac{1}{2}+\frac{1}{2}\Bigg(\sum_{j:\bm{x}_j\in D}\alpha_j k(\mathbf{x}_i,\mathbf{x}_j)+\beta\Bigg),
\end{align}}
%
%
where $c_1=\frac{\pi}{2\lambda p}$, $c_2=\frac{1}{2\lambda n}$ and $\xi_i$ is the slack variable associated with sample $\bm{x}_i\in D_n$. Notice that slack variables are used to make the objective function differentiable. 

Finally, by using vector notation,~(\ref{eq:doubleobj}) can be rewritten in a more compact form:
%
%
{\small\begin{align}
\min_{\bm{\alpha},\bm{\xi},\beta}&\:\Big\{{-}c_1\tilde{\mathbf{1}}^T\mathbf{K}\bm{\alpha}-c_1\tilde{\mathbf{1}}^T\mathbf{1}\beta+c_2\mathbf{1}_n^T\bm{\xi}+\frac{1}{2}\bm{\alpha}^T\mathbf{K}\bm{\alpha}\Big\}\nonumber\\
\text{s.t.}&\:\bm{\xi}\succeq\mathbf{0}_n,\nonumber\\
&\:\bm{\xi}\succeq\mathbf{U}\mathbf{K}\bm{\alpha}+\beta\mathbf{1}_n,\nonumber\\
&\:\bm{\xi}\succeq\frac{1}{2}\mathbf{1}_n+\frac{1}{2}\mathbf{U}\mathbf{K}\bm{\alpha}+\frac{\beta}{2}\mathbf{1}_n,\nonumber
\end{align}}
%
%

\subsection{Derivation of the dual problem}
The Lagrangian function for problem~(\ref{eq:doubleprimal}) is defined as follows:
%
%
{\small\begin{align}
\mathcal{L}(\bm{\alpha},\bm{\xi},\beta,\bm{\beta},\bm{\gamma},\bm{\delta})=&\:\frac{1}{2}\bm{\alpha}^T\mathbf{K}\bm{\alpha}-c_1\tilde{\mathbf{1}}^T\mathbf{K}\bm{\alpha}-c_1\tilde{\mathbf{1}}^T\mathbf{1}\beta+c_2\mathbf{1}_n^T\bm{\xi}\nonumber\\
&\:-\bm{\eta}^T\bm{\xi}+\bm{\gamma}^T\big(\mathbf{U}\mathbf{K}\bm{\alpha}+\beta\mathbf{1}_n-\bm{\xi}\big)\nonumber\\
&\:+\bm{\delta}^T\bigg(\frac{1}{2}\mathbf{1}_n+\frac{1}{2}\mathbf{U}\mathbf{K}\bm{\alpha}+\frac{\beta}{2}\mathbf{1}_n-\bm{\xi}\bigg)\nonumber
\end{align}}
%
%
where $\bm{\eta}\succeq\mathbf{0}_n,\bm{\gamma}\succeq\mathbf{0}_n$ and $\bm{\delta}\succeq\mathbf{0}_n$ are vectors of size $u$ containing the Lagrange multipliers associated to the constraints of the primal problem. By taking the derivatives of $\mathcal{L}$ with respect to $\bm{\alpha},\bm{\xi},\beta$ and equating them to zero, we obtain the following relations:
%
%
{\small
\begin{equation*}
\begin{array}{ll}
\frac{\partial\mathcal{L}}{\partial\bm{\alpha}}=\mathbf{0}_n &\Rightarrow\bm{\alpha}=c_1\tilde{\mathbf{1}}-\mathbf{U}^T\bm{\gamma}-\frac{1}{2}\mathbf{U}^T\bm{\delta},\\
\frac{\partial\mathcal{L}}{\partial\beta}=0&\Rightarrow c_1\tilde{\mathbf{1}}^T\mathbf{1}-\bm{\gamma}^T\mathbf{1}_n-\frac{1}{2}\bm{\delta}^T\mathbf{1}_n=0\\
&\Rightarrow \mathbf{1}^T\bigg(c_1\tilde{\mathbf{1}}-\mathbf{U}^T\bm{\gamma}-\frac{1}{2}\mathbf{U}^T\bm{\delta}\bigg)=0,\\
\frac{\partial\mathcal{L}}{\partial\bm{\xi}}=\mathbf{0}_n&\Rightarrow c_2\mathbf{1}_n-\bm{\eta}-\bm{\gamma}-\bm{\delta}=\mathbf{0}_n \wedge\:\bm{\eta},\bm{\gamma},\bm{\delta}\succeq\mathbf{0}_n\\
&\Rightarrow\bm{\gamma}+\bm{\delta}\preceq c_2\mathbf{1}_n\:\wedge\:\mathbf{0}_n\preceq\bm{\gamma},\bm{\delta}\preceq c_2\mathbf{1}_n,
\end{array}
\end{equation*}}
%
%
which are then used to build the Lagrange dual function and consequently derive the following Lagrange dual problem (we skip the derivation due to lack of space):
%
%
{\small\begin{align}
\max_{\bm{\gamma},\bm{\delta}}&\:\bigg\{{-}\frac{1}{2}\bigg(\bm{\gamma}+\frac{1}{2}\bm{\delta}\bigg)^T\mathbf{UKU}^T\bigg(\bm{\gamma}+\frac{1}{2}\bm{\delta}\bigg)+c_1\tilde{\mathbf{1}}^T\mathbf{KU}^T\bigg(\bm{\gamma}+\frac{1}{2}\bm{\delta}\bigg)\nonumber\\
&\:+\frac{1}{2}\mathbf{1}_n^T\bm{\delta}\bigg\}\nonumber\\
\text{s.t.}&\:\mathbf{1}^T\bigg[c_1\tilde{\mathbf{1}}-\mathbf{U}^T\bigg(\bm{\gamma}+\frac{1}{2}\bm{\delta}\bigg)\bigg]=0,\nonumber\\
&\:\bm{\gamma}+\bm{\delta}\preceq c_2\mathbf{1}_n,\nonumber\\
&\:\mathbf{0}_n\preceq\bm{\gamma},\bm{\delta}\preceq c_2\mathbf{1}_n,\nonumber
\end{align}}
%
%
(\ref{eq:doubledual}) can be finally derived by defining $\bm{\sigma}=\bm{\gamma}+\frac{1}{2}\bm{\delta}$ and rewriting it as a minimization problem.

==> representer.tex <==
Similarly to \cite{scholkopf2001generalized}, define $\Phi$ as the set, whose elements are the representers of the training dataset $D=D_p\cup D_n$, namely
%
%
{\small$\Psi=\big\{\varphi_{\mathbf{x}_i}\in\mathcal{H}_k|i:\bm{x}_i\in D\big\}$}.
%
%
Be $\mathcal{H}_{\Psi}$ the linear subspace of $\mathcal{H}_k$ spanned by the elements in $\Psi$ and $\bar{\mathcal{H}}_{\Psi}$ its orthogonal complement, such that $\mathcal{H}_k=\mathcal{H}_{\Psi}\oplus\bar{\mathcal{H}}_{\Psi}$:
%
%
{\small\begin{align}
\mathcal{H}_{\Psi}&=\bigg\{g\in\mathcal{H}_k|g=\sum_{i:\bm{x}_i\in D}\alpha_i\varphi_{\mathbf{x}_i},\alpha_i\in\mathbb{R}\bigg\}\nonumber\\
\bar{\mathcal{H}}_{\Psi}&=\big\{h\in\mathcal{H}_k|\langle h,g\rangle_{\mathcal{H}_k}=0,\forall g\in\mathcal{H}_{\Psi} \big\}\nonumber
\end{align}}
%
%
Therefore, any function $f\in\mathcal{H}_k$ can be decomposed in two orthogonal components, namely {\small$f=f^*+f^{\bot}$} where $f^*\in\mathcal{H}_{\Psi}$ and $f^{\bot}\in\bar{\mathcal{H}}_{\Psi}$.
Evaluating the function $f$ at the training point $\mathbf{x}_j$ is performed by exploiting the previous properties, viz.
%
%
{\small
\begin{align*}
f(\mathbf{x}_j)&=\langle\varphi_{\mathbf{x}_j},f^*+f^{\bot}\rangle_{\mathcal{H}_k}\\
&=\langle\varphi_{\mathbf{x}_j},f^*\rangle_{\mathcal{H}_k}\\
&=\langle\varphi_{\mathbf{x}_j},\sum_{i:\bm{x}_i\in D}\alpha_i\varphi_{\mathbf{x}_i}\rangle_{\mathcal{H}_k}\\
&=\sum_{i:\bm{x}_i\in D}\alpha_i\langle\varphi_{\mathbf{x}_j},\varphi_{\mathbf{x}_i}\rangle_{\mathcal{H}_k}\\
&=\sum_{i:\bm{x}_i\in D}\alpha_ik(\mathbf{x}_j,\mathbf{x}_i)\\
&=\sum_{i:\bm{x}_i\in D}\alpha_ik(\mathbf{x}_i,\mathbf{x}_j)
\end{align*}}
%
%
where the first and second equalities are due to the reproducing property of RKHS and orthogonality, respectively. The third and the fourth equalities are simple application of the inner product properties. The fifth equality holds by the definition of reproducing kernel, while the last one is valid thanks to the simmetry of any Mercer kernel. This relation highlights the fact that the evaluation of any function $f$ at any training point $\mathbf{x}_j$ is independent of $f^{\bot}$. Consequently, since $R_{emp}(f)$ is a functional of $f$ evaluated at all samples of the training dataset, we have that $R_{emp}(f)$ is also independent of $f^{\bot}$. In other words, $R_{emp}(f)=R_{emp}(f^*)$.
Furthermore, thanks to the orthogonality property, one can express the regularization term in~(\ref{eq:puopt}) in the following way:
%
%
{\small\begin{equation*}
\|f\|_{\mathcal{H}_k}^2=\|f^*+f^{\bot}\|_{\mathcal{H}_k}^2=\|f^*\|_{\mathcal{H}_k}^2+\|f^{\bot}\|_{\mathcal{H}_k}^2
\end{equation*}}
%
%
The objective function in~(\ref{eq:puopt}) can be therefore lower bounded in the following way:
%
%
{\small\begin{align}
\mathcal{R}_{emp}(f)+\lambda\|f\|_{\mathcal{H}_k}^2=&\:\mathcal{R}_{emp}(f^*)+\lambda\|f^*\|_{\mathcal{H}_k}^2+\lambda\|f^{\bot}\|_{\mathcal{H}_k}^2\nonumber\\
\geq&\:\mathcal{R}_{emp}(f^*)+\lambda\|f^*\|_{\mathcal{H}_k}^2\nonumber 
\end{align}}
%
%
which is valid for any $f\in\mathcal{H}_k$. $f^*$ is therefore the minimizer of~(\ref{eq:puopt}) and it assumes the following form:
%
%
{\small\begin{equation*}
f^*(\mathbf{x})=\sum_{i:\bm{x}_i\in D}\alpha_i\langle\varphi_{\mathbf{x}_i},\varphi_{\mathbf{x}}\rangle_{\mathcal{H}_k}=\sum_{i:\bm{x}_i\in D}\alpha_ik(\mathbf{x}_i,\mathbf{x})
\end{equation*}}
%
%
Q.E.D.


==> twovars.tex <==
\externaldocument{src/algorithm}
By introducing the following notation, namely
%
%
{\small$$\bm{\sigma}_S^k=\begin{bmatrix}
\sigma_i^k\\
\sigma_j^k
\end{bmatrix}{,}
\bm{\delta}_S^k=\begin{bmatrix}
\delta_i^k\\
\delta_j^k
\end{bmatrix}{,}
\bm{K}_{SS}={\arraycolsep=1.0pt\begin{bmatrix}
k(\bm{x}_i{,}\bm{x}_i)&k(\bm{x}_i{,}\bm{x}_j)\\
k(\bm{x}_j{,}\bm{x}_i)&k(\bm{x}_j{,}\bm{x}_j)
\end{bmatrix}}{,}
\bm{e}=\begin{bmatrix}
\bm{e}_1\\
\bm{e}_2
\end{bmatrix}
$$}
%
%
the objective function of the QP subproblem~(\ref{eq:qpsub}) evaluated at $(\bm{\sigma}_S^k,\bm{\delta}_S^k)$ can be rewritten as:
%
%
{\small\begin{equation}
\label{eq:objective}
F(\sigma_i^k,\sigma_j^k)-\frac{\delta_i^k}{2}-\frac{\delta_j^k}{2}
\end{equation}}
%
%
where
%
%
{\small\begin{align}
F(\sigma_i^k,\sigma_j^k)=&\frac{1}{2}
\begin{bmatrix}
\sigma_i^k & \sigma_j^k
\end{bmatrix}
\begin{bmatrix}
k(\bm{x}_i,\bm{x}_i) & k(\bm{x}_i,\bm{x}_j)\\
k(\bm{x}_j,\bm{x}_i) & k(\bm{x}_j,\bm{x}_j)
\end{bmatrix}
\begin{bmatrix}
\sigma_i^k \\
\sigma_j^k
\end{bmatrix}\nonumber\\
&+\begin{bmatrix}
\bm{e}_1 & \bm{e}_2
\end{bmatrix}
\begin{bmatrix}
\sigma_i^k \\
\sigma_j^k
\end{bmatrix}\nonumber
\end{align}}
%
%
and the constraints of~(\ref{eq:qpsub}) at $(\bm{\sigma}_S^k,\bm{\delta}_S^k)$ are therefore:
%
%
{\small\begin{align}
\label{eq:feasible}
&\sigma_i^k+\sigma_j^k=a^k,\nonumber\\
&\sigma_i^k+\frac{\delta_i^k}{2}\leq c_2\:\wedge\:\sigma_j^k+\frac{\delta_j^k}{2}\leq c_2,\nonumber\\
&\sigma_i^k-\frac{\delta_i^k}{2}\geq 0\:\wedge\:\sigma_j^k-\frac{\delta_j^k}{2}\geq 0,\nonumber\\
&0\leq\delta_i^k,\delta_j^k\leq c_2,
\end{align}}
%
%
where $a^k=c_1p-\bm{1}^T\bm{\sigma}_{\bar{S}}^k$ is a constant scalar for iteration $k$.

Since $(\bm{\sigma}_S^*,\bm{\delta}_S^*)$ is an optimal solution of~(\ref{eq:qpsub}), it has to satisfy the Karush-Kuhn-Tucker (KKT) conditions. In particular, the stationarity conditions can be expressed in the following way:
%
%
{\small\begin{align}
\label{eq:stationarity}
\frac{\partial\mathcal{L}}{\partial\sigma_i^k}=&
\frac{\partial F(\sigma_i^*,\sigma_j^*)}{\sigma_i^k}+\beta+\lambda_i-\mu_i=0,\nonumber\\
\frac{\partial\mathcal{L}}{\partial\sigma_j^k}=&
\frac{\partial F(\sigma_i^*,\sigma_j^*)}{\sigma_j^k}+\beta+\lambda_j-\mu_j=0,\nonumber\\
\frac{\partial\mathcal{L}}{\partial\delta_i^k}=&
{-}\frac{1}{2}+\frac{\lambda_i}{2}+\frac{\mu_i}{2}+\xi_i-\eta_i=0,\nonumber\\
\frac{\partial\mathcal{L}}{\partial\delta_j^k}=&
{-}\frac{1}{2}+\frac{\lambda_j}{2}+\frac{\mu_j}{2}+\xi_j-\eta_j=0,
\end{align}}
%
%
where $\mathcal{L}$ is the Lagrange dual function obtained from the QP subproblem and $\beta,\lambda_i,\lambda_j,\mu_i,\mu_j,\xi_i,\xi_j,\eta_i,\eta_j$ are its Lagrange multipliers, namely:
%
%
{\small\begin{align}
\mathcal{L}=&F(\sigma_i^*,\sigma_j^*)-\frac{\delta_i^*}{2}-\frac{\delta_j^*}{2}+\beta(\sigma_i^*+\sigma_j^*-a^k)\nonumber\\&
+\lambda_i(\sigma_i^*+\frac{\delta_i^*}{2}-c_2)+\lambda_j(\sigma_j^*+\frac{\delta_j^*}{2}-c_2)\nonumber\\
&-\mu_i(\sigma_i^*-\frac{\delta_i^*}{2})-\mu_j(\sigma_j^*-\frac{\delta_j^*}{2})\nonumber\\
&+\xi_i(\delta_i^*-c_2)+\xi_j(\delta_j^*-c_2)-\eta_i\delta_i^*-\eta_j\delta_j^*\nonumber
\end{align}}
%
%
%
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.3\textwidth]{img/constraints}
\vspace{-2em}
\caption{Inequality constraints of the QP subproblem~(\ref{eq:qpsub}) for a given sample $\bm{x}_i$. The coloured area corresponds to the feasible region.}
\label{fig:constraints}
\end{figure}
%
%
Now, focus on terms associated with sample $\bm{x}_i$ and specifically on its inequality constraints in~(\ref{eq:feasible}). Based on them, it is possible to distinguish the following four cases (Figure~\ref{fig:constraints} helps to understand this):
%
%
{\small\begin{align}
\label{eq:case1}
&0\leq\delta_i^k<c_2\:\wedge\:\frac{\delta_i^k}{2}<\sigma_i^k<c_2-\frac{\delta_i^k}{2},\\
\label{eq:case2}
&0\leq\delta_i^k<c_2\:\wedge\:\sigma_i^k=c_2-\frac{\delta_i^k}{2},\\
\label{eq:case3}
&0\leq\delta_i^k<c_2\:\wedge\:\sigma_i^k=\frac{\delta_i^k}{2},\\
\label{eq:case4}
&\delta_i^k=c_2\:\wedge\:\sigma_i^k=\frac{\delta_i^k}{2},
\end{align}}
%
%
By considering the KKT complementary slackness conditions together with~(\ref{eq:stationarity}), we can derive the following statements:
%
%
{\small\begin{align}
\label{eq:conditions}
\text{Case~(\ref{eq:case1})}&\Rightarrow\:\lambda_i=0,\mu_i=0,\xi_i=0,\eta_i\geq0\nonumber\\
&\Rightarrow\:\frac{\partial F(\sigma_i^*,\sigma_j^*)}{\sigma_i^k}+\beta=0\:\wedge\:\eta_i={-}\frac{1}{2},\nonumber\\
\text{Case~
(\ref{eq:case2})}&\Rightarrow\:\lambda_i\geq0,\mu_i=0,\xi_i=0,\eta_i\geq0\nonumber\\
&\Rightarrow\:\frac{\partial F(\sigma_i^*,\sigma_j^*)}{\sigma_i^k}+\beta\leq{-}1\:\wedge\:\lambda_i\geq1\:\wedge\:\eta_i\geq0\nonumber,\\
\text{Case~
(\ref{eq:case3})}&\Rightarrow\:\lambda_i=0,\mu_i\geq0,\xi_i=0,\eta_i\geq0\nonumber\\
&\Rightarrow\:\frac{\partial F(\sigma_i^*,\sigma_j^*)}{\sigma_i^k}+\beta\geq1\:\wedge\:\mu_i\geq1\:\wedge\:\eta_i\geq0,\nonumber\\
\text{Case~
(\ref{eq:case4})}&\Rightarrow\:\lambda_i\geq0,\mu_i\geq0,\xi_i\geq0,\eta_i=0,\nonumber\\
&\Rightarrow\:-1\leq\frac{\partial F(\sigma_i^*,\sigma_j^*)}{\sigma_i^k}+\beta\leq1\:\wedge\:-1\leq\lambda_i,\mu_i\leq1,
\end{align}}
%
%
The first statement in~(\ref{eq:conditions}) is clearly a contradiction, implying that condition~(\ref{eq:case1}) is not valid for KKT. In other words, any optimal solution $(\sigma_i^*,\delta_i^*)$ does not satisfy condition~(\ref{eq:case1}), but only conditions~(\ref{eq:case2})-(\ref{eq:case4}). This fact is valid $\forall\bm{x}_u\in S$ due to the symmetry of the QP subproblem~(\ref{eq:qpsub}), which concludes the proof.
